You get PADDING, everybody gets PADDING! You get privacy? Evaluating practical QUIC website fingerprinting protections for the masses

Website fingerprinting (WF) is a well-know threat to users' web privacy. New internet standards, such as QUIC, include padding to support defenses against WF. Previous work only analyzes the effectiveness of defenses when users are behind a VPN. Yet, this is not how most users browse the Internet. In this paper, we provide a comprehensive evaluation of QUIC-padding-based defenses against WF when users directly browse the web. We confirm previous claims that network-layer padding cannot provide good protection against powerful adversaries capable of observing all traffic traces. We further demonstrate that such padding is ineffective even against adversaries with constraints on traffic visibility and processing power. At the application layer, we show that defenses need to be deployed by both first and third parties, and that they can only thwart traffic analysis in limited situations. We identify challenges to deploy effective WF defenses and provide recommendations to address them.

==> parts/censoringadv.tex <==
\begin{itemize}
\item Goal of this adversary is different, they do not have access to the full trace.
\item We evaluate with X\% of a trace. 
\item Applying a padding based defense brings down the accuracy to Y.
\end{itemize}



==> parts/collection.tex <==








%\para{Trace processing for limited adversaries.}
%We process the network captures to simulate the cases of the limited adversaries.
%Combining the information from the HAR capture with the traceroute results, we first label which resources are observable by which adversary.
%Then, per adversary, in the network captures, we remove all TLS/QUIC connections that cannot be observed by the adversary.
%This filtering is based on the destination IP of each connection.
%We then use these partial network captures in the classifier.

==> parts/defense.tex <==
\section{Other defenses}

\subsection{Preventing packet grouping}

%Traffic analysis require observing a large percentage of the traffic generated when loading a web page (as we shown in \autoref{sec:limadv}).

A middlebox on the Internet will likely observe traffic from many users at the same time.
To accurately perform traffic analysis, this middlebox needs to group the traffic per client:
Previous work showed how de-interlacing traffic from overlapping webpages loading from their time/size is difficult~\citep{wang2016realistically,gong2020zero}; by extension, we suspect that preventing the adversary from isolating the traffic from one \emph{user} also significantly raises the bar for the attacker.

Isolating the traffic from one user can be achieved by a third party using the source/destination IP+port or the QUIC connection ID.
We now explore two techniques to limit the capability from an adversary to group packets belonging to the same user together.
These solutions are heuristics: isolating one user's traffic is trivial if no one else is contacting a server at a given time.

\para{IPs and ports.} There are cases in which this grouping using IPs and ports is naturally difficult: for instance, if the client is behind a large NAT, and many clients load resources from the same destination (\eg a CDN).
Even if the client is not behind a NAT (\eg because she uses IPv6), there are proposals for QUIC to hide her source IP and port (\eg masque~\citep{quic-masque} and Near-Path NAT~\citep{near-path-nat}).

\para{Connection ID.}
When the source/destination IP+port are not uniquely identifying, users can take additional counter-measures by manually rotating the \texttt{Connection ID} field present in the QUIC header.
This field is a variable-length identifier for the connection.
The client decides which \texttt{Connection ID} is used by the server, and vice-versa.
A party can ask the other to use a new connection ID through a special QUIC frame \texttt{NEW\_CONNECTION\_ID}.
By picking a new random value, it hampers the task of reassembling connection for third parties.
This frame is encrypted as part of the payload and cannot be distinguished by the adversary.
Its length is $32$ B + the variable-length \texttt{Connection ID} (a possible size is $16$B).
There is a maximum number of active connection IDs per connection, which is implementation-dependent.
However, it is possible to retire connection IDs using another $8$B frame.
By using the two frames accordingly, it is possible to rotate the \texttt{Connection ID} every packet for one direction of the connection, at a small bandwidth usage cost.
Changing the \texttt{Connection ID} require minimal book-keeping for the other party.
One disadvantage is that the client controls only one \texttt{Connection ID}, and it is unclear if a server should decide to perform a similar rotation by default.

==> parts/discussion.tex <==
\St{can combine these points with Conclusion if not long enough}
\begin{itemize}
\item We see that padding based defenses work in some cases (limited adversary), but not for a powerful adversary.
\item Timing still leaks information.
\item Order of common resources used by websites leaks information. 
\item We can protect against b and c by keeping similar order (app-layer) and adding empty packets \St{? - unsure about this part}
\item There is no one defense that works, we have to combine different techniques to protect against different adversaries.
\item QUIC also offers rotation of client IDs. This would help. But practicality issues. \St{Maybe this can be its own section/subsection}
\end{itemize}

==> parts/methodology.tex <==
\begin{figure}[t]
	\centering
	\small
	\includegraphics[width=\linewidth]{cluster150vsquic150.eps}
	\caption{Comparison of the incoming total sizes between \mixed\ and \quic. \quic\ was selected to have the same incoming total sizes as \mixed. \Ct{rethink if we want this graph at all -- maybe move to appendix. Add second quic?}}
	\vspace{-0.3cm}
	\label{fig:cluster-150-vs-quic-150}
	\vspace{-0.2cm}
\end{figure}


\label{sec:datasets}

Previous work builds datasets from top Alexa or Tranco lists. 
These top domains are typically hosted in different IPs, and thus would not be on the same anonymity set in our adversarial model.
This would only happen if the client uses a VPN, which is out of the scope of this work. 
To account for an adversary that can observe destination IPs we create new datasets using information from our collaborator CDN provider.

\para{\mixed\ dataset.} Currently, QUIC and TLS co-exist in websites.
We use the distribution of domains among IPs from our CDN provider collaborator to identify realistic anonymity sets that could be targeted by an adversary.
We resolve IP addresses and group domains by IPs.
We discard IPs that host similar sets of domains to support load balancing; IPs for which the fraction of websites that return a successful HTTP response (when queried with HTTPS) is less than $80\%$; and  IPs that host domains which are mostly aliases or copies of a single website (\eg \texttt{casino123.com, cazino132.com}).
We identify the latter by manually examining candidate groups whose domain names result a high Jaccard similarity score between their names.
From the remaining IP groups we remove duplicate websites using \texttt{CNAME} information, to avoid underestimating performance stemming from website fingerprinting attacks misclassifying these duplicates among each other. 

After all the filtering, we end up with $593'338$ M domains \Ct{do we really mean 500 million???}.
Of these, only $50k$ IPs ($8.5\%$ of the dataset) host more than $150$ domains, with one hosting as many as $56'319$ domains. 
We choose one cluster of $150$ websites for our experiments: a hard scenario for the adversary among $91.5\%$ of the IPs served by the CDN provider.
%We choose the cluster hosted on IP $35.187.82.108$. SS: Removing for now
We also run experiments with other clusters of similar size obtaining comparable results.

\para{\quicM\ and \quicS\ datasets.}
The \mixed\ dataset is TLS-heavy: only $4\%$ (std $1.7\%$) of the traffic in this dataset is over QUIC.
This results on the classifier focusing on TLS-specific features (see \autoref{sec:powadv}), preventing us from drawing meaningful conclusions about QUIC traffic's vulnerability or QUIC-oriented defenses.

A QUIC is not yet widely deployed, the IPs served by the CDN provider do not host domains that primarily use QUIC for their main page and subresources.
Following the example of Smith \etal~\citep{smith2021website}, we build QUIC-dominated datasets by crawling Alexa 1M~\citep{alexa1M}, Umbrella 1M~\citep{umbrella1m}, and Majestic 1M~\citep{majestic1M}.
We perform HAR captures\footnote{A copy of the ``Network'' tab of the Firefox Developer Tools console.} and we identify the protocols used by those websites.
We select 150 domains that primarily use QUIC.
As the total size and number of packets have long been identified as a important and stable feature for classification~\citep{dyer2012peek}, we select these websites to match the distribution of total website sizes from the \mixed\ dataset (we present the distributions in~\autoref{fig:cluster-150-vs-quic-150}).

To study the stability of website fingerprinting attacks over time, we collected two QUIC-dominated sets of traces from these domains: one in March 2021 (\quicM) and one in September 2021 (\quicS). \quicM\ has $70\%$ of all traffic over QUIC (std $3\%$).\Ct{What about \quicS??}
%We remove 404's and domains that do not load over QUIC, which leads to a filtered list of $\approx 1$M domains.

\parait{Limitation.} \Ct{we may want to revisit this with the open world}
\mixed\ and \quic\ correspond to an anonymity set at a specific point in time.
We did not evaluate how the anonymity set change over time.
To remain accurate, the adversary must retrain on new labels if the set changes.

\para{Data Collection}
To build the datasets we collect PCAP network traces from all the index pages of the domains of our two datasets.
We use Firefox 88.0 isolated on its own network namespace (using \texttt{netns}), enabling HTTP3, and disabling telemetry and auto-update settings to minimize extraneous traffic.
We record $40$\Ct{Check number} samples for each website.
For each sample, we clean the caches by creating a fresh Firefox profile. 

We extract well-formed TLS and QUIC packets from the traces.
We run our analysis on only the time and size of these packets, to avoid relying on plaintext markers\etal~\citep{smith2021website}.

==> parts/results.tex <==
\subsection{Results}
\St{
We want to show the following results:
\begin{itemize}
\item Baseline/ideal scenario: In this case, we assume that the adversary can see and process everything. We show the performance of the classifier and feature importances. We show two cases:
	\begin{itemize}
		\item One of the clusters we picked (on a single IP) - In keeping with the limitations of using lists described in Sec 4.
		\item The set with almost 100\% QUIC - Since the cluster contains lots of sites with TLS/QUIC mix, we use this on 'pure' QUIC.
	\end{itemize}
\item Adversary with partial view of the traffic. The results from the current Sec 4.3 + classifier performance on the partial views we choose.
\item Adversary with different processing capabilities on the traffic. We say that the adversary can either have full datacenter capabilities (along the lines of telco clouds) or they might be more limited. The full capabilities is represented by our baseline. We look at limited capabilities via the following strategies:
	\begin{itemize} 
	\item Sampled NetFlow - we show on unsampled netflows + sampled flows.
	\item (maybe) Sampled sFlow - why sFlow? Because it takes part of the packet instead of flows.
	\item Alternate to sampling: using Google resources: what happens when  the adversary just uses the Google flows vs non-Google flows.
	\end{itemize}	
\end{itemize}
}



\St{@Ludo: Please dump the following plots/results here:
\begin{itemize}
\item \Lr{One of the clusters (150/203) classifier performance - acc/prec/rec/f1 + feature importance}{}
\item \Lr{100\% (or was it 80\%? ) classifier performance + feature importance}{}
\item 100\% with partial view of traffic (maybe the Google AS, if you have other ASes also those) classifier performance + feature importance
\item 100\% with netflow (not sampled) classifier performance + feature importance
\item 100\% with sampled netflow at 10/100/1000 sampling rate  classifier performance + feature importance
\item 100\% with only Google flows classifier performance + feature importance
\item 100\% with only non-Google flows classifier performance + feature importance
\end{itemize}
}

\com{
	\subsection{Realistic Threat Assessment (old)}
	\vspace{0.1cm}
	\noindent We consider the following two questions:
	
	\para{What can the adversary see?} 
	We check the portion of the client traffic that passes through any middlebox owned by the adversary. We assume that the adversary can process all the traffic they see. 
	Here, the goal is to understand how the vantage point of the adversary affects their accuracy. 
	This gives an upper bound on the adversary's classification performance since we do not make assumptions on the capabilities of the middlebox. % or that the adversary might need to combine traffic that can pass through different middleboxes (owned by the adversary).
	
	We consider two adversaries:
	\begin{enumerate}
		\item an ISP adversary who sees all traffic from a client.
		This represents the best case scenario for an adversary.
		\item an AS adversary who has a partial view of the traffic, restricted to the packets passing through a particular AS.
		Such an adversary might only see some of the resources loaded by a Web page.
		%\item an IXP adversary. Adversary that owns an IXP (or multiple IXPs). This adversary has the advantage that it might see traffic from multiple ASes. It has the disadvantage that it might see lower traffic in general (since IXPs are more concentrated in their locations). \L{LB: do we use this ?}
	\end{enumerate}
	
	%In order to model each of these adversaries, we do the following:
	
	%\begin{itemize}
	%	\item  ISP adversary: This is the ideal scenario, and serves as the base scenario for comparison with other cases. The analysis will be the results of the classification over all traffic.
	%	\item AS and IXP adversary: We perform traceroutes from the client to each site. Enumerate list of resources fetched during visit. Perform traceroute for each resource. Log ASes and IXPs encountered in each traceroute. We evaluate AS/IXP that see higher and lower amounts of traffic. 
	%\end{itemize}
	
	\para{What can the adversary realistically do with the traffic it can see?}
	In the previous scenario, we assumed that the adversary can process all the traffic it sees.
	Here, we consider the scenario that an adversary might not be able to process everything that they see (limits on storage, limits on BW, limits on computation).
	
	We use the ISP adversary, but this time consider that the ISP has a bunch of middleboxes. We would look at two cases:
	
	\begin{itemize}
		\item Can the adversary fingerprint using traffic from a single realistic middlebox?
		\begin{itemize}
			\item Computation + Storage limits (how are traces processed + stored)
			\item Timing limits (How long should things be stored for, should predictions happen quickly)
			\item Look at what ML algorithms can be used (for example, deep learning might be too complex/need more data and this is not ideal for a realistic adversary.)
			\item Do we look at training/prediction/both?
		\end{itemize}
		\item Can the adversary combine flows from multiple realistic middleboxes? \St{Still thinking about this.}
	\end{itemize}
	
	Current ideas on this:
	
	\begin{itemize}
		\item We can simulate a couple of flow sampling tools on a full trace dataset to simulate how a middlebox would process the packets. Examples are: sFlow (where packets are sampled and header + some bytes of payload are stored) and netFlow (where high level flow information is extracted and that is processed)
		\item Look at work on lawful interception.
	\end{itemize}
}

\subsection{Defense}

\St{
We organize our defense section as proposing multiple options and showing which cases they would work in (as opposed to a single one-size-fits-all):
\begin{itemize}
\item Padding-based: 
	\begin{itemize}
	\item Which cases would this work in? We first show on baseline (most likely it is not ideal for it). Padding might work well in the sampled (netflows) traffic. 
	\item How to implement? QUIC has an option for this (PADDING frames) - we do simulations and maybe show one actual implementation with QUIC.
	\end{itemize}
\item Application-layer:
	\begin{itemize}
	\item Which cases would this work in? Probably in the Google case, by switching the order of resources.
	\item  How to implement? This would have to be developer guidelines when they implement applications. We can show with a test page. 
	\end{itemize}
\item Timing-based:
\begin{itemize}
	\item Which cases would this work in? This might have to be done in conjunction with padding, by introducing frames to break up timing patterns (also related to application layer).
	\item Maybe actual implementation? To be discussed.
	\end{itemize}
\item Rotation of client IDs: 
	\begin{itemize}
	\item Reference to works that talk about client IDs. Discuss feasibility.
	\item We show with simulations (unless there is a client we can modify).
	\end{itemize}
\end{itemize}
}
